A New Heuristic for Rectilinear Crossing Minimization

A new heuristic for rectilinear crossing minimization is proposed. It is based on the idea of iteratively repositioning nodes after a first initial graph drawing. The new position of a node is computed by casting rays from the node towards graph edges. Each ray receives a mark and the one with the best mark determines the new position. The heuristic has interesting performances when compared to the best competitors which can be found in classical graph drawing libraries like OGDF.

==> abstract.tex <==
% !TEX root = ./main.tex

\begin{abstract}
A new heuristic for rectilinear crossing minimization is
proposed. It is based on the idea of iteratively repositioning nodes after a first initial graph drawing.
The new position of a node is computed by casting \emph{rays}
from the node towards graph edges. Each ray receives a mark
and the one with the best mark determines the new position.

The heuristic has interesting performances when compared to
the best competitors which can be found in classical graph
drawing libraries like
% \emph{Tulip}~\cite{auber:hal-01654518} or
\emph{OGDF}~\cite{OGDF,link_OGDF}.
%\keywords{Rectilinear crossing minimization  \and Graph drawing \and Computational geometry}
\end{abstract}

